Kinematic Model of Magnetic Domain Wall Motion for Fast, High-Accuracy Simulations

Domain wall (DW) devices have garnered recent interest for diverse applications including memory, logic, and neuromorphic primitives; fast, accurate device models are therefore imperative for large-scale system design and verification. Extant DW motion models are sub-optimal for large-scale system design either over-consuming compute resources with physics-heavy equations or oversimplifying the physics, drastically reducing model accuracy. We propose a DW model inspired by the phenomenological similarities between motions of a DW and a classical object being acted on by forces like air resistance or static friction. Our proposed phenomenological model predicts DW motion within 1.2% on average compared with micromagnetic simulations that are 400 times slower. Additionally our model is seven times faster than extant collective coordinate models and 14 times more accurate than extant hyper-reduced models making it an essential tool for large-scale DW circuit design and simulation. The model is publicly posted along with scripts that automatically extract model parameters from user-provided simulation or experimental data to extend the model to alternative micromagnetic parameters.

==> Tables/fitting_parameters.tex <==
\begin{table}[b!]
%\rowcolors{2}{gray!25}{white}
    \begin{tabular}{cccccc|cccccc}
\textbf{Aex}&\textbf{Xi}&\textbf{B}$_{\mathbf{anis}}$&$\mathbf{\alpha}$&\textbf{Msat}&\textbf{W}&&&&&\textbf{drift}&\\
pJ/m&&mT&&kA/m&nm&\textbf{c$_0$}&\textbf{c$_1$}&\textbf{c$_2$}&\textbf{c$_3$}&\textbf{const}&\textbf{d$_2$}\\\hline
\rowcolor{gray!25} 11&0.01&350&0.01&1200&100&-0.327816&2.09465x$10^{-9}$&-4.07374x$10^{-20}$&3.37818x$10^{-31}$&15.833&1.18031x$10^{-12}$\\
\rowcolor{gray!25} 11&0.01&350&0.01&1200&50&-0.192543&2.0949x$10^{-9}$&-2.40119x$10^{-20}$&1.07929x$10^{-32}$&11.1333&1.47832x$10^{-12}$\\
\rowcolor{white}   11&0.01&350&0.05&1200&100&-0.0833278&4.09925x$10^{-10}$&-9.58319x$10^{-22}$&-1.02026x$10^{-32}$&4.37769&0\\
\rowcolor{white}   11&0.01&350&0.05&1200&50&-0.0159904&3.95512x$10^{-10}$&4.95345x$10^{-22}$&-2.27335x$10^{-32}$&2.29269&0\\
\rowcolor{gray!25} 11&0.01&20&0.01&795&100&-1.40044&1.28834x$10^{-8}$&-4.95528x$10^{-19}$&6.15237x$10^{-30}$&18.4994&5.07485x$10^{-12}$\\
\rowcolor{gray!25} 11&0.01&20&0.01&795&50&-0.971463&1.14437x$10^{-8}$&-3.4x$10^{-19}$&3.17481x$10^{-30}$&11.7179&4.98379x$10^{-12}$\\
\rowcolor{white}   11&0.01&20&0.05&795&100&-0.555523&2.53405x$10^{-9}$&-1.31949x$10^{-20}$&-1.07108x$10^{-31}$&3.36506&5.3368x$10^{-13}$\\
\rowcolor{white}   11&0.01&20&0.05&795&50&0.391407&1.82735x$10^{-9}$&2.01763x$10^{-20}$&-5.7328x$10^{-31}$&2.06793&0\\
\rowcolor{gray!25} 11&0.01&350&0.01&795&100&-0.349561&4.19803x$10^{-9}$&-8.01089x$10^{-20}$&5.23564x$10^{-31}$&10.9109&2.81021x$10^{-12}$\\
\rowcolor{gray!25} 11&0.01&350&0.01&795&50&-0.202931&4.08757x$10^{-9}$&-5.46606x$10^{-20}$&5.599x$10^{-32}$&8.80952&3.12571x$10^{-12}$\\
\rowcolor{white}   11&0.01&350&0.05&795&100&-0.084875&8.05477x$10^{-10}$&-7.97314x$10^{-22}$&-3.02146x$10^{-32}$&2.23956&6.21502x$10^{-14}$\\
\rowcolor{white}   11&0.01&350&0.05&795&50&-0.0452939&7.90744x$10^{-10}$&-4.27275x$10^{-22}$&-2.04638x$10^{-32}$&1.68633&0\\
\rowcolor{gray!25} 11&0.01&20&0.01&1200&100&-1.03185&5.53454x$10^{-9}$&-1.528x$10^{-19}$&1.45547x$10^{-30}$&17.3121&2.76637x$10^{-12}$\\
\rowcolor{gray!25} 11&0.01&20&0.01&1200&50&-0.499874&4.71666x$10^{-9}$&-7.04164x$10^{-20}$&8.12521x$10^{-32}$&10.8541&2.97993x$10^{-12}$\\
\rowcolor{white}   11&0.01&20&0.05&1200&100&-0.257899&1.0622x$10^{-9}$&-2.2129x$10^{-21}$&-5.09497x$10^{-32}$&3.35312&0\\
\rowcolor{white}   11&0.01&20&0.05&1200&50&-0.112976&9.09635x$10^{-10}$&-7.90319x$10^{-22}$&-2.02029x$10^{-32}$&1.94647&0\\
\rowcolor{gray!25} 11&0.05&350&0.01&1200&100&-0.325737&2.09326x$10^{-9}$&-4.06124x$10^{-20}$&3.35418x$10^{-31}$&15.8331&1.17917x$10^{-12}$\\
\rowcolor{gray!25} 11&0.05&350&0.01&1200&50&-0.177771&2.06368x$10^{-9}$&-2.23121x$10^{-20}$&-1.01067x$10^{-32}$&11.1295&1.56464x$10^{-12}$\\
\rowcolor{white}   11&0.05&350&0.05&1200&100&-0.0829628&4.09845x$10^{-10}$&-9.62696x$10^{-22}$&-1.00254x$10^{-32}$&4.37802&0\\
\rowcolor{white}   11&0.05&350&0.05&1200&50&-0.0315738&4.02452x$10^{-10}$&-9.57333x$10^{-23}$&-1.10957x$10^{-32}$&2.38663&0\\
\rowcolor{gray!25} 11&0.05&20&0.01&795&100&-1.41323&1.28887x$10^{-8}$&-4.95862x$10^{-19}$&6.1578x$10^{-30}$&18.5026&5.07242x$10^{-12}$\\
\rowcolor{gray!25} 11&0.05&20&0.01&795&50&-0.829388&1.11686x$10^{-8}$&-3.26881x$10^{-19}$&3.06865x$10^{-30}$&12.3651&5.63483x$10^{-12}$\\
\rowcolor{white}   11&0.05&20&0.05&795&100&-0.52807&2.53199x$10^{-9}$&-1.3192x$10^{-20}$&-1.06238x$10^{-31}$&3.36463&5.22352x$10^{-13}$\\
\rowcolor{white}   11&0.05&20&0.05&795&50&-0.183981&2.09662x$10^{-9}$&-3.09524x$10^{-21}$&-1.13552x$10^{-31}$&2.11406&0\\
\rowcolor{gray!25} 11&0.05&350&0.01&795&100&-0.350771&4.19901x$10^{-9}$&-8.01842x$10^{-20}$&5.24917x$10^{-31}$&10.9114&2.81251x$10^{-12}$\\
\rowcolor{gray!25} 11&0.05&350&0.01&795&50&-0.203847&4.08708x$10^{-9}$&-5.46187x$10^{-20}$&5.52447x$10^{-32}$&8.80973&3.12473x$10^{-12}$\\
\rowcolor{white}   11&0.05&350&0.05&795&100&-0.0842591&8.05293x$10^{-10}$&-7.89853x$10^{-22}$&-3.02889x$10^{-32}$&2.2395&5.93041x$10^{-14}$\\
\rowcolor{white}   11&0.05&350&0.05&795&50&-0.0456227&7.90809x$10^{-10}$&-4.33767x$10^{-22}$&-2.0275x$10^{-32}$&1.68626&0\\
\rowcolor{gray!25} 11&0.05&20&0.01&1200&100&-1.10622&5.57442x$10^{-9}$&-1.55548x$10^{-19}$&1.50208x$10^{-30}$&17.34&2.77631x$10^{-12}$\\
\rowcolor{gray!25} 11&0.05&20&0.01&1200&50&-0.500256&4.71751x$10^{-9}$&-7.0505x$10^{-20}$&8.30021x$10^{-32}$&10.8539&2.98049x$10^{-12}$\\
\rowcolor{white}   11&0.05&20&0.05&1200&100&-0.247743&1.05838x$10^{-9}$&-1.99707x$10^{-21}$&-5.41455x$10^{-32}$&3.35194&0\\
\rowcolor{white}   11&0.05&20&0.05&1200&50&-0.11241&9.09464x$10^{-10}$&-7.79534x$10^{-22}$&-2.03844x$10^{-32}$&1.94643&0\\
\rowcolor{gray!25} 31&0.01&350&0.01&1200&100&-0.617235&3.76184x$10^{-9}$&-7.80547x$10^{-20}$&5.55483x$10^{-31}$&17.0611&1.88905x$10^{-12}$\\
\rowcolor{gray!25} 31&0.01&350&0.01&1200&50&-0.315081&3.59307x$10^{-9}$&-3.09407x$10^{-20}$&-2.9066x$10^{-31}$&10.7475&2.2543x$10^{-12}$\\
\rowcolor{white}   31&0.01&350&0.05&1200&100&-0.137465&7.23643x$10^{-10}$&-1.07336x$10^{-21}$&-2.68309x$10^{-32}$&3.74649&2.45171x$10^{-13}$\\
\rowcolor{white}   31&0.01&350&0.05&1200&50&-0.0579012&7.01421x$10^{-10}$&-7.08905x$10^{-23}$&-1.61259x$10^{-32}$&2.01573&0\\
\rowcolor{gray!25} 31&0.01&20&0.01&795&100&-5.34956&2.32919x$10^{-8}$&-1.01487x$10^{-18}$&1.28124x$10^{-29}$&15.2213&4.08656x$10^{-12}$\\
\rowcolor{gray!25} 31&0.01&20&0.01&795&50&-2.32512&1.90917x$10^{-8}$&-4.89393x$10^{-19}$&5.76884x$10^{-31}$&11.2106&4.99156x$10^{-12}$\\
\rowcolor{white}   31&0.01&20&0.05&795&100&-1.50753&4.46256x$10^{-9}$&-2.27988x$10^{-20}$&-2.51574x$10^{-31}$&3.2785&8.25196x$10^{-13}$\\
\rowcolor{white}   31&0.01&20&0.05&795&50&-0.492361&3.64466x$10^{-9}$&-4.47854x$10^{-21}$&-2.33985x$10^{-31}$&2.09555&0\\
\rowcolor{gray!25} 31&0.01&350&0.01&795&100&-0.663281&7.31999x$10^{-9}$&-1.88687x$10^{-19}$&1.66393x$10^{-30}$&14.2347&3.86679x$10^{-12}$\\
\rowcolor{gray!25} 31&0.01&350&0.01&795&50&-0.415096&7.10858x$10^{-9}$&-1.2829x$10^{-19}$&4.64709x$10^{-31}$&10.8722&4.42356x$10^{-12}$\\
\rowcolor{white}   31&0.01&350&0.05&795&100&-0.139774&1.38308x$10^{-9}$&-1.83303x$10^{-21}$&-6.84219x$10^{-32}$&2.69529&7.73346x$10^{-13}$\\
\rowcolor{white}   31&0.01&350&0.05&795&50&-0.0604238&1.34747x$10^{-9}$&-4.44672x$10^{-22}$&-5.0214x$10^{-32}$&1.89959&1.40105x$10^{-13}$\\
\rowcolor{gray!25} 31&0.01&20&0.01&1200&100&-2.55491&1.02828x$10^{-8}$&-2.68604x$10^{-19}$&1.82734x$10^{-30}$&15.6142&3.25055x$10^{-12}$\\
\rowcolor{gray!25} 31&0.01&20&0.01&1200&50&-0.999123&8.33623x$10^{-9}$&-9.1783x$10^{-20}$&-8.84412x$10^{-31}$&9.91666&3.21129x$10^{-12}$\\
\rowcolor{white}   31&0.01&20&0.05&1200&100&-0.535442&1.9473x$10^{-9}$&-2.24827x$10^{-21}$&-1.12425x$10^{-31}$&2.97517&0\\
\rowcolor{white}   31&0.01&20&0.05&1200&50&-0.182993&1.61503x$10^{-9}$&-2.15265x$10^{-22}$&-4.76001x$10^{-32}$&1.74943&0\\
\rowcolor{gray!25} 31&0.05&350&0.01&1200&100&-0.617264&3.7621x$10^{-9}$&-7.80746x$10^{-20}$&5.55912x$10^{-31}$&17.0594&1.88784x$10^{-12}$\\
\rowcolor{gray!25} 31&0.05&350&0.01&1200&50&-0.315097&3.59348x$10^{-9}$&-3.09759x$10^{-20}$&-2.90009x$10^{-31}$&10.7464&2.25343x$10^{-12}$\\
\rowcolor{white}   31&0.05&350&0.05&1200&100&-0.14033&7.24528x$10^{-10}$&-1.12699x$10^{-21}$&-2.59746x$10^{-32}$&3.74633&2.46096x$10^{-13}$\\
\rowcolor{white}   31&0.05&350&0.05&1200&50&-0.0583918&7.01767x$10^{-10}$&-9.27123x$10^{-23}$&-1.57813x$10^{-32}$&2.01548&0\\
\rowcolor{gray!25} 31&0.05&20&0.01&795&100&-5.34939&2.32917x$10^{-8}$&-1.01475x$10^{-18}$&1.2807x$10^{-29}$&15.2238&4.08404x$10^{-12}$\\
\rowcolor{gray!25} 31&0.05&20&0.01&795&50&-2.31314&1.90854x$10^{-8}$&-4.88741x$10^{-19}$&5.59434x$10^{-31}$&11.205&4.98721x$10^{-12}$\\
\rowcolor{white}   31&0.05&20&0.05&795&100&-1.49988&4.46161x$10^{-9}$&-2.27365x$10^{-20}$&-2.52683x$10^{-31}$&3.28072&8.33114x$10^{-13}$\\
\rowcolor{white}   31&0.05&20&0.05&795&50&-0.484501&3.64294x$10^{-9}$&-4.38821x$10^{-21}$&-2.35365x$10^{-31}$&2.09622&0\\
\rowcolor{gray!25} 31&0.05&350&0.01&795&100&-0.663205&7.3195x$10^{-9}$&-1.88637x$10^{-19}$&1.66291x$10^{-30}$&14.2357&3.86809x$10^{-12}$\\
\rowcolor{gray!25} 31&0.05&350&0.01&795&50&-0.413961&7.10639x$10^{-9}$&-1.28119x$10^{-19}$&4.6163x$10^{-31}$&10.8741&4.42542x$10^{-12}$\\
\rowcolor{white}   31&0.05&350&0.05&795&100&-0.14725&1.38501x$10^{-9}$&-1.95724x$10^{-21}$&-6.62817x$10^{-32}$&2.6954&7.61023x$10^{-13}$\\
\rowcolor{white}   31&0.05&350&0.05&795&50&-0.06001&1.34736x$10^{-9}$&-4.40157x$10^{-22}$&-5.02552x$10^{-32}$&1.89942&1.47166x$10^{-13}$\\
\rowcolor{gray!25} 31&0.05&20&0.01&1200&100&-2.58103&1.02945x$10^{-8}$&-2.6951x$10^{-19}$&1.84549x$10^{-30}$&15.6321&3.25411x$10^{-12}$\\
\rowcolor{gray!25} 31&0.05&20&0.01&1200&50&-0.999485&8.33616x$10^{-9}$&-9.17699x$10^{-20}$&-8.8472x$10^{-31}$&9.91771&3.21147x$10^{-12}$\\
\rowcolor{white}   31&0.05&20&0.05&1200&100&-0.534434&1.94696x$10^{-9}$&-2.22389x$10^{-21}$&-1.12904x$10^{-31}$&2.9753&0\\
\rowcolor{white}   31&0.05&20&0.05&1200&50&-0.182747&1.61497x$10^{-9}$&-2.11309x$10^{-22}$&-4.76681x$10^{-32}$&1.74944&0\\
    \end{tabular}
\end{table}
